Towards Secure and Decentralized Sharing of IoT Data

The Internet of Things (IoT) bears unprecedented security and scalability challenges due to the magnitude of data produced and exchanged by IoT devices and platforms. Some of those challenges are currently being addressed by coupling IoT applications with blockchains. However, current blockchain-backed IoT systems simply use the blockchain to store access control policies, thereby underutilizing the power of blockchain technology. In this paper, we propose a new framework named Sash that couples IoT platforms with blockchain that provides a number of advantages compared to state of the art. In Sash, the blockchain is used to store access control policies and take access control decisions. Therefore, both changes to policies and access requests are correctly enforced and publicly auditable. Further, we devise a ``data marketplace'' by leveraging the ability of blockchains to handle financial transaction and providing ``by design'' remuneration to data producers. Finally, we exploit a special flavor of identity-based encryption to cater for cryptography-enforced access control while minimizing the overhead to distribute decryption keys. We prototype Sash by using the FIWARE open source IoT platform and the Hyperledger Fabric framework as the blockchain back-end. We also evaluate the performance of our prototype and show that it incurs tolerable overhead in realistic deployment settings.

==> applications.tex <==
\section{Application: IoT Search}
\label{sec:application}

IoT search system refers to an engine that is connected to multiple IoT systems (domains) to index and crawl IoT data up on requests from users of the engine. Multiple domains where the search engine connects do not hold pre-trust established relationships. However, they are supposed to comply with sets of policies on sharing data when they are connected to the search engine. In this system, we define two levels for data sharing rules: global rules and domain-local rules. The global data sharing policies are ones that all domains contractually agree on. For example, ``No data owner can give consumer access to their data to terrorist group or embargo countries''. The domain-local policies are onces that each individual domain creates to restrict access to their data. In this system, only validated policies are executed. Also a domain policy once validated is modified only if it gets approval by the network and it cannot revoke an proved policy without requiring new approval on the removal. 

The system described thus far instantiates a policy decision point on the blockchain and ensures the correct evaluation of a policy via consensus. Nevertheless, the policy decision is still enforced at the platform. In other words, correct enforcement of a policy relies on the trustworthiness of the platform that ultimately decides whether to grant or deny a request to access data. Further, the platform sees clear-text data as produced by devices. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{policy.pdf}
    \caption{Policy management for Inter-Domain in IoTSearch.}
    \label{fig:policy}
\end{figure}

Mapping our data sharing scheme to inter-domain policy management, we consider policies are special data that must be advertised and approved by the blockchain network. A domain once created a policy can advertise it on the network and wait for approval (offer acceptance in our sharing scheme). Global policies also can be initiated by a node and approved by other nodes. Validate policies are visible to any nodes so that they can verify if an actual data sharing comply to such policies. Policy enforcement is made via the blockchain such that only valid sharing actions i.e. update ACL and distribute decryption keys are executed by respective smart contracts.   


==> ourporposal.tex <==

\section{Data Marketplace and Sharing Schemes}

\subsection{Data Marketplace}

In our system context, a ``data marketplace'' $\market$ allows IoT data owners to create data offer by advertising the data (or a piece of data) over the blockchain and data consumers to accept the offer. The data offer is implemented in smart contract and executed on the blockchain network. The data consumer, once accepted the offer and made the payment (if that is a condition in data offer), can get access to the data. We design three functions over $\market$: \textbf{add} data, \textbf{create} data offer and \textbf{accept} offer.

Algorithm.~\ref{algo:adddata} describes a smart contract for adding a data to the market. The data is verified before added. As the actual data is store in the cloud $\cloud$, the meta-data offered over the blockchain $\blockchain$ should be corresponding to that of data on $\cloud$. A check \texttt{VerifyData()} is done before the data is added. The main check is done for existence of the data in storage and its signature signed by $\owner$ is valid. We assume public key of $\owner$ to verify the signature is known by other parties.

Algorithm.~\ref{algo:offer} describes smart contracts for adding a data offer to the market $\market$ and for accepting an existing offer followed by a payment. 

\SetKwProg{Fn}{Function}{}{}

{\SetAlgoNoLine%
\begin{algorithm}[]
 \KwData{$\owner$, data $d$, signature $sig$, blockchain $\blockchain$}
 \KwResult{adds $d$ to the data market $\market$ }
 map: key-value stored on $\blockchain$\;

 \Fn{VerifyData ($\owner$, $d$)}{
 \ForAll{files in $d$}{
 \If{(files do not exist in the cloud) or (file id in the cloud different than submitted file id) or (owner in the cloud different than user) or (cloud ACL different than file ACL)}{return false}

 }
 return true\;
 }

\Fn{AddData ($\owner$, $d$, $sig$)}{
\If{signature not valid}{return error}
\If{!VerifyData($d$, $\owner$)}{return error}
\If{$d$ already exists}{return error}
key = "data"||$d$.filesID\;
map.Set(key, $d$)\;
return success\;
 }
 \caption{Add data to data market}
 \label{algo:adddata}   

\end{algorithm}
}

{\SetAlgoNoLine%
\begin{algorithm}[]
 \KwData{$\owner$, offer $ofr$, signature $sig$}
 \KwResult{adds $offer$ to the data market $\market$}
 map: key-value stored on the blockchain $\blockchain$\;

 \Fn{OfferCreate ($\owner$, $ofr$, $sig$)}{
 \If{signature not valid}{return error}

 \If{!VerifyData($offer$.data, $\owner$)}{return error}
$offer$.state = true\;
key = "offer"||data.ID\;
 map.Set(key,offer)\;
 return success\;
 }

\Fn{OfferAccept (user, offer, sign)}{
\If{signature not valid}{return error}
\If{!offer.state}{return error}
\If{!VerifyData(offer.data,offer.data.owner)}{return error}
\If{data already exists}{return error}
offer.state = false\;
key = "offer"||data.ID\;
 map.Set(key,offer)\;
 \eIf{user.ID > offer.data.owner}{
key = "IOU"||hash(user.ID,offer.data.owner)\;
value = GetCurrentIOUValue(key)+offer.value\;
 }{
 key = "IOU"||hash(offer.data.owner,user.ID)\;
value = GetCurrentIOUValue(key)-offer.value\;
 }
map.Set(key,value)\;
key = "data"||offer.data.ID\;
map.set(key,Append(offer.data.ACL,user.ID)\;
return success\;
 }
 \caption{Offer and Purchase data}
 \label{algo:offer}
\end{algorithm}
}


\subsection{Data sharing with ACL}
\label{sec:proposal:acl}

Access Control List (ACL) is a straightforward technique to manage data sharing in a sense who can access what on a data resource. In ACL-based scheme, a data owner stores its data on a storage either locally or on a remote cloud and access to such data is handled via ACL. Figure~\ref{fig:acl} depicts our design that leverages blockchain to form a ``data market'' where data provider and data consumer can advertise the data $d$ to share and accept offer on such data. The data offer is described in smart contract form and run on the blockchain network. The data consumer, once accepted the offer and made the payment (if that is a condition in data offer), will appear in updated ACL of the data item $d$. ACL is replicated by all nodes of the network. In this design, the cloud storage participate in the network as a node and it keeps synchronization with latest versions of ACL. The data consumer after the completion of payment transaction can download the data $d$ from the cloud.

The benefit of using ACL over blockchain for handling data sharing is the removal of a trusted authority to maintain the ACL. Instead, ACL is replicated by nodes and all transactions are verified and made visible (transparent) to all nodes.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{sharing-ACL2.pdf}
    \caption{Data sharing scheme using ACL.}
    \label{fig:acl}
\end{figure}



\subsection{Data sharing with IBE}
\label{sec:proposal:ibe}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{sharing-IBE2.pdf}
    \caption{Data sharing scheme using IBE.}
    \label{fig:ibe}
\end{figure}
In this section we introduce Identity Based Encryption (IBE)~\cite{xxx} as a cryptographic mechanism that allows to forego the trust assumption on the platform. By using IBE, the platform no longer sees cleartext data nor it enforces any policy.

Prefix encryption is particularly suited for IoT scenarios where a multitude of devices are organized in a hierarchy. Further, no global key-distribution authority is needed as the owner of a set of devices may act as the authority to distribute keys to decrypt ciphertext generated by its own devices. For example, Alice may organize her IoT devices in an hierarchical namespace \texttt{alice.}, including \texttt{alice.house.} for devices installed at her house and \texttt{alice.car.} for devices installed in her car. Alice can thus create her own master key-pair (i.e., by running $Setup(1^\lambda)$) and load the master public key on her devices. Each device will produce data encrypted under its own ``name''. For example, the smart thermostat may encrypt its measurement $m$ via $Encrypt(mpk,\texttt{alice.home.thermostat},m)$ and upload the ciphertext to the platform. Envelope encryption may be used to encrypt bulk data.



Distribution of secret keys to eligible parties is achieved by smart contract that Alice deploys  on the blockchain and an application running at her premises that handles the master secret key $msk$. The smart contract receives requests to obtain secret keys for a specific device name (e.g., \texttt{alice.home.thermostat}) or for a set of devices (e.g., \texttt{alice.home.}), and evaluates whether to grant or deny the request. If the request is granted, the smart contract invokes the application running at Alice's premises that runs $Extract$ to compute the secret decryption key and securely transfer that key to the requestor. Note that requests carry the public key of the requestor so that the application extracting secret keys can securely transfer those keys to the intended party.



Once a party obtains a decryption key associated to the name of a given device, it can ask for data produced by that device to the platform. The platform does not manage cleartext data as devices only upload encrypted data. Therefore, the platform does not carry out any policy enforcement but simply forwards the ciphertexts uploaded by the device in the request to the requestor. Finally the requestor holding runs the $Decrypt$ algorithm and recovers the cleartext data. Note a requestor may use the decryption key for a set of devices (e.g., \texttt{alice.home.}) to decrypt ciphertext produced by any device in that set (e.g., \texttt{alice.home.thermostat} or \texttt{alice.home.doorlock}).

Fig.~\ref{fig:ibe} shows our IBE-based data sharing scheme. Similar to ACL-based scheme, data offer and offer acceptance are done over the blockchain via executions of smart contracts. The difference of this scheme compared to ACL-based scheme is how data is stored and shared. Data producers instead of storing clear data as in ACL-based scheme, they encrypt their data before uploading it to the cloud. Data consumers, with proper transactions have been done, can retrieve the encrypted data and decryption key to compute clear data. The Key Manager handles key distribution. It does not require to be an independent entity but can be integrated to existing component such as Identity Manager component that is necessary to maintain the membership of nodes in the blockchain.

\subsection{Integration to IoT platform FIWARE}
\label{sec:proposal:integration}

Among state-of-the-art IoT platforms, we chose FIWARE to demonstrate how our proposal can be integrated to an IoT platform. To extend FIWARE with our private data sharing scheme, we introduce two handlers Blockchain Handler and Domain Router which direct flow of data between the two parts (Fig.\ref{fig:integration}). In this particular design, we consider IoT Domain, a virtual concept for a group of IoT stakeholders that share common settings (e.g. located in a same building, produce same type of context data), as a node that plays roles of data producer and data consumer. This IoT Domain can be referred as IoT middleware layer component which provides capabilities to connect to further systems and applications that low-level IoT hardware-based components lack of. Each IoT Domain maintains a Broker to forward communications from IoT stakeholders to further applications.

When IoT stakeholders connect to their IoT Domain, the respective Broker will route the data stream to a right handler. More specifically, IoT data uploads will be directed to Cloud Data Storage. Queries on retrieving data from the IoT to do a particular physical action by IoT stakeholders will depend on permissions assigned on such requested data. Here IoT Domains join the blockchain network and establish data sharing transactions over it. As we have introduced two sharing schemes, having an ACL or a key manager is adjustable in this integration. Similarly, whether or not that the cloud storage joins the blockchain network (data market) is also adjustable, without any required changes on architecture of existing IoT platforms. We argue that our proposals can be integrated to other IoT platforms with proper adjustments.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{integration.pdf}
    \caption{Integration to FIWARE.}
    \label{fig:integration}
\end{figure}




==> problem.tex <==
\section{Challenges}
\hien{for Hien to edit}
